PCR: Proxy-based Contrastive Replay for Online Class-Incremental Continual Learning

Online class-incremental continual learning is a specific task of continual learning. It aims to continuously learn new classes from data stream and the samples of data stream are seen only once, which suffers from the catastrophic forgetting issue, i.e., forgetting historical knowledge of old classes. Existing replay-based methods effectively alleviate this issue by saving and replaying part of old data in a proxy-based or contrastive-based replay manner. Although these two replay manners are effective, the former would incline to new classes due to class imbalance issues, and the latter is unstable and hard to converge because of the limited number of samples. In this paper, we conduct a comprehensive analysis of these two replay manners and find that they can be complementary. Inspired by this finding, we propose a novel replay-based method called proxy-based contrastive replay (PCR). The key operation is to replace the contrastive samples of anchors with corresponding proxies in the contrastive-based way. It alleviates the phenomenon of catastrophic forgetting by effectively addressing the imbalance issue, as well as keeps a faster convergence of the model. We conduct extensive experiments on three real-world benchmark datasets, and empirical results consistently demonstrate the superiority of PCR over various state-of-the-art methods.

==> PaperRebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}


% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks,bookmarks=false]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\cvprPaperID{9169} % *** Enter the CVPR Paper ID here
% \def\confName{CVPR}
% \def\confYear{2023}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{PCR: Proxy-based Contrastive Replay for Online Class-Incremental Continual Learning}  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix

% %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW

% \noindent We thank all reviewers. We are encouraged that they found 1) our work clearly explains motivation (R\#1 and R\#2). 2) our method is new (R\#3), interesting (R\#1), simple (R\#1 and R\#2), and significant (R\#1 and R\#2). 

% \vspace{-2ex}
% \section{Response to R\#1}
% \vspace{-1ex}



% %-------------------------------------------------------------------------

% % \subsection{Reply to Q1}
% \noindent\textbf{[Reply to Q1] The contribution or novelty of our work is sufficient.} First and foremost, comparative analysis of existing studies (page 3 and 4) clearly shows their limitations, providing solid motivation for us. Besides, PCR is a new coupling method but not a fine-grained improvement over ER-ACE. In addition to more reasonable mask operation, repeated anchor-to-sample pairs are the core of PCR. And it can further produce other variants (i.e., ER+A+B+C in Table 3). Last but not least, different from existing studies reporting forgetting rate, we explore the accuracy in both new and old classes, respectively. It proves that PCR is more advanced in balancing novel and historical knowledge.


% %------------------------------------------------------------------------

% % \subsection{Reply to Q2}
% \noindent\textbf{[Reply to Q2] The usage of data augmentation is fair for all methods in Table 1.} In SCR (not PCR), 10 original samples can produce 10 augmented samples, hence the number of forward passes in network is actually 20. To be fair, we concatenate 10 original samples and 10 augmented samples into a new batch containing 20 samples for other methods (lines 6/7 of Algorithm 1), including PCR and ER-ACE.

% Meahwhile, we conduct experiments on PCR and ER-ACE without data augmentation in Table~\ref{table:aug}. And additional results for ER+A on all benchmarks are shown as Table~\ref{table:ablation}.

% \begin{table}[h]
% \renewcommand\tabcolsep{3pt}
% \centering
% \vspace{-1ex}
% \caption{Final Accuracy Rate of ER-ACE and PCR on Split CIFAR100 when they do not use data augmentation.}
% \vspace{-2ex}
% \label{table:aug}
% \begin{tabular}{l|cccc}
% \hline
% Buffer Size  & 500 & 1000 & 2000 & 5000 \\ \hline
% ER-ACE      & 15.6\scriptsize±0.8  & 17.9\scriptsize±0.7  & 19.9\scriptsize±0.9  & 24.4\scriptsize±0.8   \\ \hline
% PCR     & 15.7\scriptsize±0.7  & 18.4\scriptsize±0.6  & 22.1\scriptsize±0.7  & 26.7\scriptsize±0.7  \\ \hline
% \end{tabular}
% \vspace{-3ex}
% \end{table}


% \begin{table}[h]
% \renewcommand\tabcolsep{3pt}
% \centering
% \vspace{-2ex}
% \caption{Final Accuracy Rate of ER+A on all benchmarks. The memory buffer for Split CIFAR10 is \{100, 200, 500, 1000\}}
% \vspace{-2ex}
% \label{table:ablation}
% \begin{tabular}{l|cccc}
% \hline
% Buffer Size  & 500 & 1000 & 2000 & 5000 \\ \hline
% Split CIFAR10      & 39.4\scriptsize±3.2  & 48.8\scriptsize±1.1  & 52.3\scriptsize±1.7  & 53.9\scriptsize±3.4   \\ \hline
% Split CIFAR100     & 20.5\scriptsize±0.9  & 25.5\scriptsize±0.6  & 26.0\scriptsize±0.7  & 28.2\scriptsize±0.7  \\ \hline
% Split MiniImageNet & 19.4\scriptsize±1.3  & 22.7\scriptsize±0.8  & 25.6\scriptsize±1.1  & 27.5\scriptsize±1.0   \\ \hline
% \end{tabular}
% \vspace{-3ex}
% \end{table}

% %------------------------------------------------------------------------


% \noindent\textbf{[Replay to Q3] We add an additional ablation study about batch size. } As demonstrated in Figure~\ref{fig:batch}, with the increase of batch size, PCR consistently maintains its advantages, and the gap is basically stable.

% \begin{figure}[h]
% \centering
% \vspace{-2ex}
% \includegraphics[scale=0.18]{PaperSections/PaperFigures/pcr_batch.pdf}
% \vspace{-2ex}
% \caption{Final accuracy rate of ER, ER-ACE, and PCR by different size of batch.}
% \label{fig:batch}%
% \vspace{-2ex}
% \end{figure}
% %------------------------------------------------------------------------


% \noindent\textbf{[Replay to Q4] We include NCM to other baselines.} SCR in Table 1 is based on NCM classifier, and the performance of ER-ACE+NCM is described as Table~\ref{table:acencm}. 


% \begin{table}[h]
% \renewcommand\tabcolsep{3pt}
% \centering
% \vspace{-2ex}
% \caption{Final Accuracy Rate of ER-ACE+NCM on all benchmarks. The buffer for Split CIFAR10 is \{100, 200, 500, 1000\}}
% \vspace{-2ex}
% \label{table:acencm}
% \begin{tabular}{l|cccc}
% \hline
% Buffer Size  & 500 & 1000 & 2000 & 5000 \\ \hline
% Split CIFAR10      & 45.0\scriptsize±1.3  & 51.0\scriptsize±1.2  & 56.8\scriptsize±1.1  & 60.1\scriptsize±1.0   \\ \hline
% Split CIFAR100     & 21.0\scriptsize±0.6  & 24.2\scriptsize±0.7  & 26.6\scriptsize±0.7  & 29.1\scriptsize±1.0  \\ \hline
% Split MiniImageNet & 18.1\scriptsize±0.8  & 22.3\scriptsize±0.5  & 25.3\scriptsize±0.5  & 27.1\scriptsize±0.9   \\ \hline
% \end{tabular}
% \vspace{-2ex}
% \end{table}

% %------------------------------------------------------------------------
% \vspace{-2ex}
% \section{Response to R\#2} 
% \vspace{-2ex}
% %-------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q1/Q3] We will improve Figure 1 and 2 to make them easier to understand.} Thanks for comment.

% %------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q2] We report cumulative gradients of proxies.} As shown in Figure~\ref{fig:gradient}, PCR produces uniform gradient distribution for all proxies.

% \begin{figure}[h]
% \centering
% \vspace{-2ex}
% \includegraphics[scale=0.18]{PaperSections/PaperFigures/pcr_gradient.pdf}
% \vspace{-3ex}
% \caption{Cumulative gradients of different methods when model learns new classes(9/10) on Split CIFAR10.}
% \label{fig:gradient}%
% \vspace{-3ex}
% \end{figure}


% %------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q4] NCM classifier is more suitable for situation with smaller image and larger buffer.} Small-sized images are easy to obtain reliable features, and large-sized buffer trends to obtain accurate classification centers.
% %------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q5] PCR keeps fast convergence of proxy-based replay manners.} Its convergence rate is similar with ER, SS-IL and ER-ACE (3.3), but faster than SCR (3.4).
% %------------------------------------------------------------------------


% \vspace{-2ex}
% \section{Response to R\#3} 
% \vspace{-2ex}

% %-------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q1/Q2] We will explain proxy and PCR.} A proxy can be regarded as the representative of a sub-dataset. PCR replaces anchor-to-sample pairs with anchor-to-proxy pairs in contrastive loss, while [38] adds anchor-to-sample pairs to anchor-to-proxy pairs in cross-entropy loss.

% %------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q3/Q4] SS-IL and OCM will be contained in Table 1, but their absence does not affect the progressiveness of PCR.} On the one hand, detailed analysis of SS-IL can be found in [6]. And its performance on online CICL is far from ER-ACE. On the other hand, the experimental setup of OCM is different from that in our work. OCM retrieves 100 samples from buffer for each step. Meanwhile, it is trained by Adam optimizer with 0.001 learning rate. Moreover, based on its source code, we find that OCM does not shuffle the class indexes for each run. Hence, we conduct additional experiments on Split CIFAR100 (Table 3) for fair comparison. Moreover, as the latest method, ER-ACE and ER-DVC in Table 1 are also defeated by PCR. All of results are enough to show the competitiveness of PCR.



% %------------------------------------------------------------------------

% \noindent\textbf{[Replay to Q5/Q6] PCR is efficient for running and can be straightly extended to deal with fuzzy task boundary.}


% %------------------------------------------------------------------------
% % In fact, NCM is useful but not necessary for PCR. As it needs to perform additional forward calculation, which affects its practicability in online settings.



% % %%%%%%%%% REFERENCES
% % {\small
% % \bibliographystyle{ieee_fullname}
% % \bibliography{egbib}
% % }

% \end{document}

